Keep Your Friends Close: Leveraging Affinity Groups to Accelerate AI Inference Workflows

AI inference workflows are typically structured as a pipeline or graph of AI programs triggered by events. As events occur, the AIs perform inference or classification tasks under time pressure to respond or take some action. Standard techniques that reduce latency in other streaming settings (such as caching and optimization-driven scheduling) are of limited value because AI data access patterns (models, databases) change depending on the triggering event: a significant departure from traditional streaming. In this work, we propose a novel affinity grouping mechanism that makes it easier for developers to express application-specific data access correlations, enabling coordinated management of data objects in server clusters hosting streaming inference tasks. Our proposals are thus complementary to other approaches such as caching and scheduling. Experiments confirm the limitations of standard techniques, while showing that the proposed mechanism is able to maintain significantly lower latency as workload and scale-out increase, and yet requires only minor code changes.

==> sections/90-workload.tex <==

Figure~\ref{fig:videos_actors}
show the workload of each video (\little, \hyang, and \gates), as well as the
aggregated workload for two simultaneous videos (\littlehyang), and three
simultaneous videos (\littlehyanggates).  Workload is expressed in number of
actors detected in each frame. It is possible to see that \little has the lowest
workload across all 700 frames, while \gates has the highest -- during the first
half of the videos, there are more actors in \gates frames than in the
aggregated \littlehyang frames.

\begin{figure}[h]
    \centering
    % [trim={left bottom right top},clip]
    \includegraphics[width=0.6\linewidth,clip,trim={0.4cm 0.45cm 0.35cm 0.35cm}]{plot/cameras_workload.pdf}
    \caption{Number of actors for different workloads.}
    \label{fig:videos_actors}
\end{figure}

Figure~\ref{fig:mot_state_size}
shows the size of the MOT state (in MBs) for each frame of each of the three
videos employed in our experiments.

\begin{figure}[h]
    \centering
    % [trim={left bottom right top},clip]
    \includegraphics[width=0.6\linewidth,clip,trim={0.4cm 0.45cm 0.35cm 0.35cm}]{plot/mot_state_size.pdf}
    \caption{Size of the MOT state for each frame of each video.}
    \label{fig:mot_state_size}
\end{figure}


